Inducing Sparsity and Shrinkage in Time-Varying Parameter Models

Time-varying parameter (TVP) models have the potential to be over-parameterized, particularly when the number of variables in the model is large. Global-local priors are increasingly used to induce shrinkage in such models. But the estimates produced by these priors can still have appreciable uncertainty. Sparsification has the potential to reduce this uncertainty and improve forecasts. In this paper, we develop computationally simple methods which both shrink and sparsify TVP models. In a simulated data exercise we show the benefits of our shrink-then-sparsify approach in a variety of sparse and dense TVP regressions. In a macroeconomic forecasting exercise, we find our approach to substantially improve forecast performance relative to shrinkage alone.

==> Results/lps_table_large.tex <==
% latex table generated in R 3.5.2 by xtable 1.8-3 package
% Mon Apr 22 17:24:55 2019
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrrrrrrr}
  \hline
 & DL & LASSO & NG & horse & SSVS & DL & LASSO & NG & horse & SSVS \\ 
  \hline
LPS & 38.82 & 17.64 & 46.56 & 89.85 & 6.33 & 80.73 & 50.19 & 72.84 & 134.30 & 21.46 \\ 
  X1 & 5.06 & 3.37 & 13.94 & 25.33 & -3.35 & 26.66 & 27.37 & 30.37 & 43.74 & 7.10 \\ 
  X12 & 19.17 & 17.87 & 18.37 & 21.39 & 13.60 & 23.50 & 18.05 & 17.19 & 20.43 & 14.28 \\ 
  X15 & 15.82 & -1.44 & 16.61 & 47.87 & -2.78 & 34.10 & 7.96 & 27.10 & 75.61 & 1.57 \\ 
  LPS.1 & 159.17 & 128.00 & 220.81 & 331.69 & 52.20 & 294.32 & 253.68 & 309.17 & 403.25 & 135.88 \\ 
  X1.1 & 63.04 & 54.21 & 95.22 & 140.44 & 23.77 & 127.27 & 119.41 & 144.62 & 181.82 & 61.45 \\ 
  X12.1 & 67.37 & 61.62 & 88.59 & 111.46 & 35.15 & 101.79 & 91.28 & 100.64 & 114.17 & 58.09 \\ 
  X15.1 & 58.33 & 34.94 & 74.73 & 139.04 & 9.41 & 112.84 & 77.15 & 110.09 & 175.74 & 35.90 \\ 
   \hline
\end{tabular}
\end{table}


==> Results/lps_table_medium.tex <==
% latex table generated in R 3.5.2 by xtable 1.8-3 package
% Mon Apr 22 19:29:41 2019
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrrrrrrr}
  \hline
 & DL & LASSO & NG & horse & SSVS & DL & LASSO & NG & horse & SSVS \\ 
  \hline
LPS & 21.27 & 5.12 & 28.81 & 40.90 & 4.88 & 45.36 & 35.66 & 51.10 & 57.58 & 29.74 \\ 
  X1 & 0.85 & -3.32 & 2.11 & 4.97 & -2.19 & 14.34 & 15.76 & 15.14 & 16.08 & 11.17 \\ 
  X6 & 2.68 & -0.99 & 2.67 & 4.77 & 0.08 & 4.13 & 0.29 & 2.49 & 1.10 & 2.30 \\ 
  X8 & 18.09 & 8.95 & 24.17 & 31.78 & 6.85 & 28.37 & 21.35 & 34.95 & 42.65 & 17.28 \\ 
  LPS.1 & 5.13 & -18.02 & 14.21 & 24.69 & -16.49 & 32.93 & 33.37 & 36.04 & 34.04 & 25.23 \\ 
  X1.1 & -5.20 & -16.57 & -2.07 & 2.26 & -12.88 & 15.78 & 17.70 & 16.78 & 16.91 & 13.09 \\ 
  X6.1 & 1.38 & -6.21 & 3.27 & 6.09 & -4.90 & 4.61 & 4.39 & 4.58 & 3.05 & 3.20 \\ 
  X8.1 & 6.46 & -3.09 & 11.51 & 17.20 & -5.20 & 17.64 & 17.31 & 20.54 & 21.26 & 12.80 \\ 
   \hline
\end{tabular}
\end{table}


==> Results/lps_table_small.tex <==
% latex table generated in R 3.5.2 by xtable 1.8-3 package
% Mon Apr 22 17:28:08 2019
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrrrrrrr}
  \hline
 & DL & LASSO & NG & horse & SSVS & DL & LASSO & NG & horse & SSVS \\ 
  \hline
LPS & 13.50 & 3.70 & 13.90 & 14.47 & 8.23 & 15.65 & 9.80 & 16.85 & 17.34 & 13.18 \\ 
  X1 & 0.59 & -2.39 & 0.30 & -0.33 & -0.76 & 1.90 & 1.80 & 1.46 & 1.48 & 0.69 \\ 
  X2 & -1.37 & -3.21 & -2.09 & -2.07 & -1.99 & -3.20 & -5.60 & -3.63 & -4.88 & -3.35 \\ 
  X3 & 14.99 & 9.48 & 16.06 & 17.40 & 11.14 & 18.21 & 15.26 & 20.22 & 22.52 & 17.07 \\ 
  LPS.1 & 7.33 & 1.33 & 7.14 & 8.75 & 4.58 & 5.38 & 2.68 & 5.45 & 6.59 & 4.77 \\ 
  X1.1 & 1.61 & -1.22 & 1.22 & 0.99 & 0.53 & 2.89 & 4.56 & 3.18 & 3.38 & 2.37 \\ 
  X2.1 & 0.25 & -0.14 & -0.15 & 0.61 & 0.16 & -0.94 & -1.45 & -1.37 & -1.42 & -1.27 \\ 
  X3.1 & 5.92 & 0.89 & 6.40 & 7.39 & 3.28 & 5.98 & 4.23 & 7.01 & 8.63 & 5.47 \\ 
   \hline
\end{tabular}
\end{table}


==> Results/rmse_table_large.tex <==
% latex table generated in R 3.5.2 by xtable 1.8-3 package
% Mon Apr 22 17:24:55 2019
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrrrrrrr}
  \hline
 & DL & LASSO & NG & horse & SSVS & DL & LASSO & NG & horse & SSVS \\ 
  \hline
X1 & 0.72 & 0.61 & 0.64 & 0.59 & 0.72 & 0.46 & 0.42 & 0.46 & 0.38 & 0.57 \\ 
  X12 & 0.77 & 0.88 & 0.88 & 0.78 & 0.92 & 0.70 & 0.88 & 0.89 & 0.72 & 0.93 \\ 
  X15 & 0.43 & 0.74 & 0.55 & 0.44 & 0.61 & 0.34 & 0.71 & 0.53 & 0.38 & 0.59 \\ 
  X1.1 & 0.12 & 0.12 & 0.09 & 0.07 & 0.17 & 0.09 & 0.09 & 0.08 & 0.08 & 0.13 \\ 
  X12.1 & 0.15 & 0.18 & 0.22 & 0.16 & 0.18 & 0.15 & 0.17 & 0.21 & 0.15 & 0.16 \\ 
  X15.1 & 0.06 & 0.10 & 0.21 & 0.06 & 0.09 & 0.05 & 0.07 & 0.17 & 0.05 & 0.08 \\ 
   \hline
\end{tabular}
\end{table}


==> Results/rmse_table_medium.tex <==
% latex table generated in R 3.5.2 by xtable 1.8-3 package
% Mon Apr 22 19:29:41 2019
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrrrrrrr}
  \hline
 & DL & LASSO & NG & horse & SSVS & DL & LASSO & NG & horse & SSVS \\ 
  \hline
X1 & 1.11 & 1.14 & 1.12 & 1.07 & 1.16 & 0.84 & 0.84 & 0.84 & 0.84 & 0.88 \\ 
  X6 & 0.96 & 1.00 & 0.97 & 0.94 & 1.00 & 0.97 & 1.01 & 0.98 & 0.99 & 0.99 \\ 
  X8 & 0.98 & 1.07 & 0.99 & 0.96 & 1.05 & 0.90 & 0.99 & 0.92 & 0.91 & 0.97 \\ 
  X1.1 & 1.04 & 1.03 & 1.05 & 1.00 & 1.06 & 0.93 & 0.91 & 0.93 & 0.93 & 0.94 \\ 
  X6.1 & 0.99 & 1.00 & 1.00 & 0.98 & 0.99 & 1.00 & 1.00 & 0.99 & 0.99 & 1.00 \\ 
  X8.1 & 0.94 & 1.03 & 0.94 & 0.90 & 1.04 & 0.89 & 0.88 & 0.86 & 0.85 & 0.94 \\ 
   \hline
\end{tabular}
\end{table}


==> Results/rmse_table_small.tex <==
% latex table generated in R 3.5.2 by xtable 1.8-3 package
% Mon Apr 22 17:28:08 2019
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrrrrrrr}
  \hline
 & DL & LASSO & NG & horse & SSVS & DL & LASSO & NG & horse & SSVS \\ 
  \hline
X1 & 1.00 & 1.04 & 1.00 & 1.01 & 1.01 & 1.01 & 1.02 & 1.01 & 1.03 & 1.02 \\ 
  X2 & 1.03 & 1.06 & 1.04 & 1.04 & 1.04 & 1.06 & 1.09 & 1.07 & 1.08 & 1.06 \\ 
  X3 & 1.01 & 1.05 & 1.02 & 1.02 & 1.04 & 0.99 & 1.00 & 1.00 & 1.00 & 1.00 \\ 
  X1.1 & 0.95 & 0.97 & 0.95 & 0.95 & 0.95 & 1.02 & 1.01 & 1.02 & 1.02 & 1.03 \\ 
  X2.1 & 1.01 & 1.02 & 1.01 & 1.01 & 1.01 & 1.02 & 1.02 & 1.02 & 1.02 & 1.01 \\ 
  X3.1 & 0.92 & 0.94 & 0.91 & 0.90 & 0.94 & 0.94 & 0.91 & 0.91 & 0.92 & 0.94 \\ 
   \hline
\end{tabular}
\end{table}

